Towards Automated Continuous Security Compliance

Context: Continuous Software Engineering is increasingly adopted in highly regulated domains, raising the need for continuous compliance. Adherence to especially security regulations -- a major concern in highly regulated domains -- renders Continuous Security Compliance of high relevance to industry and research. Problem: One key barrier to adopting continuous software engineering in the industry is the resource-intensive and error-prone nature of traditional manual security compliance activities. Automation promises to be advantageous. However, continuous security compliance is under-researched, precluding an effective adoption. Contribution: We have initiated a long-term research project with our industry partner to address these issues. In this manuscript, we make three contributions: (1) We provide a precise definition of the term continuous security compliance aligning with the state-of-art, (2) elaborate a preliminary overview of challenges in the field of automated continuous security compliance through a tertiary literature study, and (3) present a research roadmap to address those challenges via automated continuous security compliance.

==> sections/00_abstract.tex <==
\textbf{Context:} Continuous Software Engineering is increasingly adopted in highly regulated domains, raising the need for continuous compliance. Adherence to especially security regulations -- a major concern in highly regulated domains -- renders \emph{Continuous Security Compliance} of high relevance to industry and research. 

\textbf{Problem:} One key barrier to adopting continuous software engineering in the industry is the resource-intensive and error-prone nature of traditional manual security compliance activities. Automation promises to be advantageous. However, continuous security compliance is under-researched, precluding an effective adoption.

\textbf{Contribution:} We have initiated a long-term research project with our industry partner to address these issues. In this manuscript, we make three contributions: (1) We provide a precise definition of the term continuous security compliance aligning with the state-of-art, (2) elaborate a preliminary overview of challenges in the field of automated continuous security compliance through a tertiary literature study, and (3) present a research roadmap to address those challenges via automated continuous security compliance.
